FootstepNet: an Efficient Actor-Critic Method for Fast On-line Bipedal Footstep Planning and Forecasting

Designing a humanoid locomotion controller is challenging and classically split up in sub-problems. Footstep planning is one of those, where the sequence of footsteps is defined. Even in simpler environments, finding a minimal sequence, or even a feasible sequence, yields a complex optimization problem. In the literature, this problem is usually addressed by search-based algorithms (e.g. variants of A*). However, such approaches are either computationally expensive or rely on hand-crafted tuning of several parameters. In this work, at first, we propose an efficient footstep planning method to navigate in local environments with obstacles, based on state-of-the art Deep Reinforcement Learning (DRL) techniques, with very low computational requirements for on-line inference. Our approach is heuristic-free and relies on a continuous set of actions to generate feasible footsteps. In contrast, other methods necessitate the selection of a relevant discrete set of actions. Second, we propose a forecasting method, allowing to quickly estimate the number of footsteps required to reach different candidates of local targets. This approach relies on inherent computations made by the actor-critic DRL architecture. We demonstrate the validity of our approach with simulation results, and by a deployment on a kid-size humanoid robot during the RoboCup 2023 competition.

==> discussion.tex <==
\section{Discussion} \label{discuss}

==> related_work.tex <==
\section{Related Work} \label{RW}

% Optimization-based approaches
Kanoun \textit{et al.} \cite{kanoun2011planning} proposed to formulate the footstep planning an as
inverse kinematics problem. The footsteps sequence is represented by an equivalent
kinematic chain, where each footstep is made of two prismatic joints and a revolute joint.
Such a problem can be solved iteratively by a gradient descent, which suffers from
inevitable convergence to local optimum.
\textbf{TODO: Plus de méthodes optimization-based}

% Search-based
\textbf{TODO: Expliquer le concept des méthodes search-based}
\textbf{TODO: Citer d'autre travaux, comme D* ou ARA (le temps est prohibitif)}
A faster search-based approach was proposed by Missura and Bennewitz \cite{missura2021fast}.
In this work, the shortest path is included in the heuristic function in order to abort the search prematurely. 
The authors present a replanning rate of 50Hz, by limiting the computation time to 18ms.
However, other heuristics like the rotate-translate-rotate (RTR) are explicitely added to the formulation.
Even if natural, RTR is still arbitrary and might result in suboptimal behaviour. 
The performance is obtained with assumptions which heavily restricts the considered alternatives.

% RL (whole-body)
Some DRL-based work address the locomotion problem in an end-to-end manner.
Lee \textit{et al.} \cite{lee2020learning} proposed a controller for quadruped robot to
navigate on challenging terrains, and deployed on real robots using only proprioceptive information.
Haarnoja \textit{et al.} \cite{haarnoja2023learning} demonstrated impressive soccer skills on bipedal robots,
by using exteroceptive ground-truth for state estimation.
Footstep planning is here not considered explicitely, but an inherent result of the whole controllers.
This choice of architecture come with complex reward shaping and costly trainings.
Designed for specific tasks, they also arguably lack of versatility and modularity.

% RL (footstep)
\textbf{TODO: Citer DeepQ ?}
Hofer and Rouxel \cite{hofer2017operational} proposed a RL-based approach to produce walk orders to approach a soccer
ball. However, they didn't consider obstacles.
Tsounis \textit{et al.} \cite{tsounis2020deepgait}, quadrupedal locomotion is separated in two DRL subproblems: the Gait Planner (GP) and Gait Controller.
GP addresses a geometrical problem which is the quadruped-equivalent of the footstep planning. Even if feasibility
is extensively checked at this stage, it is unclear that the reward function encourages a minimization of the number
of steps because of its complexity.

